Cinderella User's Manual

{\sc Cinderella} is a software solution for the quantitative comparison of time series in the frequency domain. It assigns probabilities to coincident peaks in the DFT amplidude spectra of the datasets under consideration. Two different modes are available. In conditional mode, {\sc Cinderella} examines target and comparison datasets on the assumption that the latter contain artifacts only, returning the conditional probability of a target signal, although there is a coincident signal in the comparison data within the frequency resolution. In composed mode, the probability of coincident signal components in both target and comparison data is evaluated. {\sc Cinderella} permits to examine multiple target and comparison datasets at once.

==> CoAst_layo.tex <==
\pagestyle{fancyplain}
\addtolength{\headwidth}{\marginparsep}
\addtolength{\headwidth}{\marginparwidth}
\addtolength{\headwidth}{\marginparwidth}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markright{#1}}
\lhead[\fancyplain{}{\sffamily\thepage}]{\fancyplain{}{\sffamily}}
\rhead[\fancyplain{}{\sffamily\leftmark}]{\fancyplain{}{\sffamily\thepage}}
%\rfoot[]{\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}}
%\lfoot[\fancyplain{}{\sffamily\small Communications in Asteroseismology, No. 131, July 2001}]{}
\cfoot{}
%\paperheight=230mm
%\paperwidth=150mm
\hoffset=-1cm
\voffset=1mm
\topmargin=-12mm
\headheight=5mm
\headwidth=115mm
\headsep=7mm
\oddsidemargin=1mm
\evensidemargin=1mm
\marginparwidth=0cm
\marginparsep=0cm
\renewcommand{\headrulewidth}{0pt}
\textwidth=115mm
\textheight=165mm
\footskip=10mm
\newcommand{\apj}{ApJ}
\newcommand{\aj}{AJ}  %************Stimmts?
\newcommand{\aap}{A\&A}  %*************Stimmts?
\newcommand{\mnras}{MNRAS}
\newcommand{\tspace}{\hspace{1.2em}}
\newcommand{\feh}{$[Fe/H]$}
\newcommand{\by}{\ensuremath{(b-y)}}       % b-y index
\newcommand{\nr}{\multicolumn{-1}{c}{\ensuremath{\lesssim 25}}}
\newcommand{\dss}{$\delta$~Scuti stars}                     % Style for Delta Scuti Stars (plur.)
\newcommand{\ds}{$\delta$~Scuti star}
\newcommand{\ngc}[1]{NGC~{#1}}                              % Style for NGCxxxx
\newcommand{\templogg}{\texttt{templogg}}                   % Style for "templogg" program name
\newcommand{\teff}{\ensuremath{T_{eff}}}             % T_eff
\newcommand{\logg}{\ensuremath{\log g}}                     % log g
\newcommand{\vsini}{\ensuremath{v\sin i}}                   % v sin 
\newcommand{\halpha}{H$\alpha$}  % H alpha
\def\kms {km~s$^{-1}$}
\def\kmss {km~s$^{-1}$~}
\def\cd {d$^{-1}$}

\newcommand{\kopf}{\small\itshape Comm. in Asteroseismology\\ 2008, in preparation}
\newcommand{\Authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\authors}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\renewcommand{\author}[1]{\begin{center}\normalsize\bf\sf #1 \end{center}}
\newcommand{\Address}[1]{\begin{center}\small\sf #1 \end{center}}
\newcommand{\address}[1]{\begin{center}\small\sf #1 \end{center}}
\renewenvironment{abstract}{\section*{Abstract}\normalsize\sf}{}
\newcommand{\References}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}
%\newcommand{\references}[1]{\begin{flushleft}{\large References\\}\vspace*{2mm}\small #1 \end{flushleft}}

\newcommand{\chapterDSSN}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headDSSN}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\chapterdssn}[2]{\chapter[\sf\normalsize #1\\ \footnotesize \hspace*{5mm}by #2 \sf\normalsize][]{#1\\}\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\headdssn}[2]{\rhead[\fancyplain{}{\sf\footnotesize \center{#1}}]{\fancyplain{}{\sffamily\thepage}}\lhead[\fancyplain{\kopf}{\sffamily\thepage}]{\fancyplain{\kopf}{\sf\footnotesize \center{#2}}}}

\newcommand{\figureDSSN}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand{\figuredssn}[5]{\begin{figure}[#4]
\centering
\includegraphics*[#5]{#1}
\caption{#2}
\label{#3}
\end{figure}}
\newcommand {\strich} {\begin{center} \vspace{0.5cm} \rule{1.5cm}{0.3mm} \end{center}}
\renewcommand{\chaptername}{}
\newcommand{\acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgments}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}
\newcommand{\Acknowledgements}[1]{\vspace*{5mm}\noindent\begin{bf}Acknowledgments. \end{bf} #1}


==> caput_coast.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge CoAst  \\ Announcements \\
\end{center}



==> caput_editorialcomment.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}



\section*{Editorial statement for the following paper (entitled \\ {\it MOST found evidence for solar-type oscillations in the K2 giant star HD\,20884)} }
{\it \small The main message of the following paper is to report the detection of nonradial pulsation in a K giant. This is an important and controversial topic.

A key issue for this investigation is the reliability of the extracted frequencies. Your editor has spent his life with Fourier amplitude spectra of high-precision ground-based photometry. From that experience, Figure 3 of the paper
represents the natural result of instrumental instabilities and atmospheric transparency changes and does not deserve a second look. However, these are satellite observations without the typical ground-based difficulties -- but there may be different problems.

The statistical analyses can only help us in a limited way. It does not matter much whether one applies my favorite criterion of amplitude signal/noise ratio < 4, the SigSpec values, or another method. All these statistical analyses rely on assumptions of the nature of noise present in the data. Again, in ground-based photometry, we have found that the statistics are not reliable for low-frequency peaks. The obvious method to verify that certain peaks are not noise is to look at a comparison sample: the authors provide the results for another star with a simpler light curve. In my opinion, the issue is not yet solved.\normalsize}




==> caput_empty.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
%here would come some text

\end{center}



==> caput_helas.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 

\newpage 

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge HELAS  \\ News \\
\end{center}



==> caput_papers.tex <==


%%Version 1: this style won't cause trouble while compiling. it gives the name of the section and the stiff sheet
%\newpage
%\lhead[\fancyplain]{\fancyplain{}{}} \rhead[\fancyplain]{\fancyplain{}{}}
%\sectionheading{News \& Announcements}
%\newpage


%%Version 2: this will only give the stiff sheet. the section heading in the TOC has to be inserted with the command given below. Yet this will cause trouble when compiling the masterfile.
%\addtocontents{toc}{\vspace{1cm} \large\textbf{Recent Communications} \vspace{0cm} \normalsize} 


\newpage 

\pagenumbering{arabic}%
\setcounter{page}{1}%
%von mir geändert von 0 auf 1

\thispagestyle{empty}
\vspace*{30mm}
\begin{center}
\huge Scientific  \\ Papers \\
\end{center}


\newcounter{paper} 
\stepcounter{paper}
\def\code{P}
%\renewcommand\thepage {\code\arabic{paper}-\arabic{page} } 

%\newcounter{paperpage}
%\stepcoutner{paperpage}{page}
%\thepage


%\stepcounter{paper}

%\newcommand\thepapercode{\code\thepaper-\thepage}

